Limits and Colimits in the Category of Pastures

We show that the category of pastures has arbitrary limits and colimits of diagrams indexed by a small category.

==> Ref.tex <==
%Category Theory for the Working Mathematician
@book{mac2013categories,
  title={Categories for the working mathematician},
  author={Mac Lane, Saunders},
  volume={5},
  year={2013},
  publisher={Springer Science \& Business Media}
}

%moduli space of matroids
@article{baker2018moduli,
  title={The moduli space of matroids},
  author={Baker, Matthew and Lorscheid, Oliver},
  journal={arXiv preprint arXiv:1809.03542},
  year={2018}
}

%Foundations of matroids
@article{baker2020foundations,
  title={Foundations of matroids I: Matroids without large uniform minors},
  author={Baker, Matthew and Lorscheid, Oliver},
  journal={arXiv preprint arXiv:2008.00014},
  year={2020}
}

%Descartes Rule of Signs and Newton Polygons
@article{baker2021descartes,
  title={Descartes' rule of signs, Newton polygons, and polynomials over hyperfields},
  author={Baker, Matthew and Lorscheid, Oliver},
  journal={Journal of Algebra},
  volume={569},
  pages={416--441},
  year={2021},
  publisher={Elsevier}
}
